Two-Loop Scattering Amplitudes: Double-Forward Limit and Colour-Kinematics Duality

We propose new formulae for the two-loop n-point D-dimensional integrands of scattering amplitudes in Yang-Mills theory and gravity. The loop integrands are written as a double-forward limit of tree-level trivalent diagrams, and are inferred from the formalism of the two-loop scattering equations. We discuss the relationship between the formulae for non-supersymmetric theories and the Neveu-Schwarz sector of the formulae for maximally supersymmetric theories, which can be derived from ambitwistor strings. An important property of the loop integrands is that they are expressed in a representation that includes linear-type propagators. This representation exhibits a loop-level version of the colour-kinematics duality, which follows directly from tree level via the double-forward limit.

==> 2loopvacuum.tex <==
\begin{tikzpicture}

\node[circle, draw=black, thick, fill=white, minimum size=1cm] at (1,0) {};
\node[circle, draw=black, thick, fill=white, minimum size=0.5cm] at (3,0) {};
\node[circle, draw=black, thick, fill=white, minimum size=0.5cm] at (4,0) {};

\draw[thick] (1,0.5) -- (1,-0.5);
\draw[thick] (3.25,0) -- (3.75,0);


\end{tikzpicture}
